Maintaining Natural Image Statistics with the Contextual Loss

Maintaining natural image statistics is a crucial factor in restoration and generation of realistic looking images. When training CNNs, photorealism is usually attempted by adversarial training (GAN), that pushes the output images to lie on the manifold of natural images. GANs are very powerful, but not perfect. They are hard to train and the results still often suffer from artifacts. In this paper we propose a complementary approach, that could be applied with or without GAN, whose goal is to train a feed-forward CNN to maintain natural internal statistics. We look explicitly at the distribution of features in an image and train the network to generate images with natural feature distributions. Our approach reduces by orders of magnitude the number of images required for training and achieves state-of-the-art results on both single-image super-resolution, and high-resolution surface normal estimation.

==> app.tex <==
\section{Applications}

In this section we present two applications:  single-image super-resolution, and high-resolution surface normal estimation.
We chose the first to highlight the advantage of using our approach in concert with GAN.
The second was selected since its output is not an image, but rather a surface of normals. This shows the generic nature of our approach to other domains apart from image generation.

To the best of our knowledge this is the first use of the Contextual loss for image restoration, prior to our work people mainly focus on L2 loss, perceptual loss, and adversarial loss. 

To asses the contribution of our suggested framework for image restoration we experiment on single-image super-resolution. 
To place our efforts in context we start by briefly reviewing some of the recent works on super-resolution. A more comprehensive overview of the current trends can be found in~\cite{timofte2017NTIRE,agustsson2017div2k}. 

Recent solutions based on CNNs can be categorized into two groups.
The first group relies on the $L2$ or $L1$ losses~\cite{ledig2016photo,LapSRN,Lim2017edsr,tong2017image}, which lead to high PSNR and SSIM~\cite{wang2004image} at the price of low perceptual quality, as was recently shown in~\cite{blau2017perception,zhang2018unreasonable}. 
The second group of works aim at high perceptual quality.
This is done by adopting perceptual loss functions~\cite{johnson2016perceptual}, sometimes in combination with GAN~\cite{ledig2016photo} or by adding the Gram loss~\cite{gatys2016image}, which nicely captures textures~\cite{sajjadi2017enhancenet}.

\input{fig_normal_data.tex}

The framework we propose is by no means limited to networks that generate images. It is a generic approach that could be useful for training networks for other tasks, where the natural statistics of the target should be exhibited in the network's output.
To support this, we present a solution to the problem of surface normal estimation -- an essential problem in computer vision, widely used for scene understanding and new-view synthesis. 
%====================================================
\subsection{Proposed solution:}


Our main goal is to generate natural looking images, with natural internal statistics.
At the same time, we do not want the structural similarity to be overly low (the trade-off between the two is nicely analyzed in~\cite{blau2017perception,zhang2018unreasonable}).   
Therefore, we propose an objective that considers both, with higher importance to perceptual quality. 
Specifically, we integrate three loss terms:
(i) The Contextual loss -- to make sure that the internal statistics of the generated image are similar to those of the ground-truth high-resolution image.
(ii) The $L2$ loss, computed at \textbf{low} resolution -- to drive the generated image to share the spatial structure of the target image. 
(iii) Finally, following~\cite{ledig2016photo} we add an adversarial term, which helps in pushing the generated image to look ``real''. 

Given a low-resolution image $s$ and a target high-resolution image $y$, our objective for training the network $G$ is:
%
\begin{equation}
\mathcal{L}(G) = \lambda_{\text{CX}}\cdot\mathcal{L}_{\text{CX}}(G(s),y) + \lambda_{{L2}}\cdot ||G(s)^{\text{LF}}-y^{\text{LF}}||_2 +\lambda_{\text{GAN}}\cdot\mathcal{L}_{\text{GAN}}(G(s))
\end{equation}
%
where in all our experiments $\lambda_{\text{CX}}\!=\!0.1$, $\lambda_{\text{GAN}}\!=\!1e-3$, and $\lambda_{{L2}}\!=\!10$.
The images $G(s)^{\text{LF}},y^{\text{LF}}$ are low-frequencies obtained by convolution with a Gaussian kernel of width $21\!\times\!21$ and $\sigma\!=\!3$. For the Contextual loss feature extraction we used layer $conv3\_4$ of VGG19~\cite{simonyan2014very}.

We propose using an objective based on a combination of three loss terms:
(i) The Contextual loss -- to make sure that the internal statistics of the generated normal map match those of the target normal map.
(ii) The $L2$ loss, computed at \textbf{low} resolution, and (iii) The $L1$ loss. Both drive the generated normal map to share the spatial layout of the target map.  
Our overall objective is:
%
\begin{equation}
\label{eq:normal-loss}
\mathcal{L}(G) = \lambda_{\text{CX}}\cdot\mathcal{L}_{\text{CX}}(G(s),y) + \lambda_{{L2}}\cdot ||G(s)^{\text{LF}}-y^{\text{LF}}||_2 + \lambda_{L1}\cdot ||G(s)-y||_1
\end{equation}
%
where, $\lambda_{\text{CX}}\!=\!1$, and $\lambda_{{L2}}\!=\!0.1$. The normal-maps $G(s)^{\text{LF}},y^{\text{LF}}$ are low-frequencies obtained by convolution with a Gaussian kernel of width $21\!\times\!21$ and $\sigma=3$. 
We tested with both $\lambda_{L1}\!=\!1$ and $\lambda_{L1}\!=\!0$, which removes the third term.


%====================================================
\subsection{Implementation details}
For the task of SR We adopt the SRGAN architecture~\cite{ledig2016photo}\footnote{We used the implementation in \url{https://github.com/tensorlayer/SRGAN}}
and train it on only 800 images from the DIV2K dataset~\cite{agustsson2017div2k}, for 1500 epoch. Our network is initialized by first training using only the $L2$ loss for 100 epochs.  

For the task of normal estimation we chose as architecture the Cascaded Refinement Network (CRN)~\cite{chen2017photographic} originally suggested for label-to-image and was shown to yield great results in a variety of other tasks~\cite{mechrez2018contextual}. 
For the contextual loss we took as features $5\!\times\!5$ patches of the normal map (extracted with stride 2) and layers $conv1\_2, conv2\_2$ of VGG19. In our implementation we reduced memory consumption by random sampling of all three layers into $65\!\times\!65$ features.

We used TensorFlow~\cite{abadi2016tensorflow} and Adam optimizer~\cite{kingma2014adam} with the default parameters ($\beta_1=0.9, \beta_2=0.999, \epsilon=1e-08$).


%====================================================
\subsection{Evaluation}

\paragraph{\textbf{Super Resolution:} \ \ \ }
Empirical evaluation was performed on the BSD100 dataset~\cite{martin2001database}.
As suggested in~\cite{blau2017perception} we compute both structural similarity (SSIM~\cite{wang2004image}) to the ground-truth and perceptual quality (NRQM~\cite{ma2017learning}).
The ``ideal'' algorithm will have both scores high.

Table~\ref{fig:SR_table} compares our method with three recent solutions whose goal is high perceptual quality. 
It can be seen that our approach outperforms the state-of-the-art on both evaluation measures.
This is especially satisfactory as we needed only $800$ images for training, while previous methods had to train on tens or even hundreds of thousands of images.
%
\input{fig_SR_table.tex}

\input{fig_SR_results.tex}


Figure~\ref{fig:SR_results} further presents a few qualitative results, that highlight the gap between our approach and previous ones.
Both SRGAN~\cite{ledig2016photo} and EnhanceNet~\cite{sajjadi2017enhancenet} rely on adversarial training (GAN) in order to achieve photo-realistic results.
This tends to over-generate high-frequency details, which make the image look sharp, however, often these high-frequency components do not match those of the target image. 
The Contextual loss, when used in concert with GAN, reduces these artifacts, and results in natural looking image patches.

An interesting observation is that we achieve high perceptual quality while using for the Contextual loss features from a mid-layer of VGG19, namely $conv3\_4$.
This is in contrast to the reports in~\cite{ledig2016photo} that had to use for SRGAN the high-layer $conv5\_4$ for the perceptual loss (and failed when using low-layer such as $conv2\_2$).
Similarly, EnhanceNet required a mixture of $pool2$ and $pool5$.



%====================================================
\paragraph{\textbf{Normal Estimation:} \ \ \ }
%\paragraph{\textbf{Data:}\ \ \ }
The task we pose is to estimate the underlying normal map from a single monocular color image. Although this problem is ill-posed, recent CNN based approaches achieve satisfactory results ~\cite{bansal2017pixelnet,wang2015designing,eigen2015predicting,wang2014multi,chen2017surface} on the NYU-v2 dataset~\cite{silbermanECCV12NYU}. 
%
Thanks to its size, quality and variety, NYU-v2 is intensively used as a test-bed for predicting depth, normals, segmentation etc.
However, due to the acquisition protocol, its data does not include the fine details of the scene and misses the underlying high frequency information, hence, it does not provide a detailed representation of natural surfaces.

Therefore, we built a new dataset of images of surfaces and their corresponding normal maps, where fine details play a major role in defining the surface structure. 
Examples are shown in Figure~\ref{fig:normal_data}.
Our dataset is based on 182 different textures and their respective normal maps that were collected from the Internet\footnote{\href{www.poliigon.com}{www.poliigon.com} and \href{www.textures.com}{www.textures.com}}, originally offered for usages of realistic interior home design, gaming, arts, etc.
For each texture we obtained a high resolution color image ($1024\!\times\!1024$) and a corresponding normal-map of a surface such that its underlying plane normal points towards the camera (see Figure~\ref{fig:normal_data}). 
Such image-normals pairs lack the effect of lighting, which plays an essential role in normal estimation.
Hence, we used Blender\footnote{\href{www.blender.org}{www.blender.org}}, a 3D renderer, to simulate each texture under $10$ different point-light locations. This resulted in a total of $1820$ pairs of image-normals.
The textures were split into $90\%$ for training and $10\%$ for testing, such that the test set includes all the $10$ rendered pairs of each included texture.

The collection offers a variety of materials including wood, stone, fabric, steel, sand, etc., with multiple patterns, colors and roughness levels, that capture the appearance of real-life surfaces. 
While some textures are synthetic, they look realistic and exhibit imperfections of real surfaces, which are translated into the fine-details of both the color image as well as its normal map.







Table~\ref{fig:normal_table} compares our results with previous solutions.
We compare to the recently proposed PixelNet~\cite{bansal2017pixelnet}, that presented state-of-the-art results on NYU-v2. 
Since PixelNet was trained on NYU-v2, which lacks fine details, we also tried fine-tuning it on our dataset. 
In addition, we present results obtained with CRN~\cite{chen2017photographic}.
While the original CRN was trained with both $L1$ and the perceptual loss~\cite{johnson2016perceptual}, this combination provided poor results on normal estimation.
Hence, we excluded the perceptual loss and report results with only $L1$ as the loss, or when using our objective of Eq.~\eqref{eq:normal-loss}.
It can be seen that CRN trained with our objective (with $L1$) leads to the best quantitative scores.
%
\input{fig_normal_table.tex}
%
\input{fig_rendered_texture.tex}

We would like to draw your attention to the inferior scores obtained when removing the $L1$ term from our objective (i.e., setting $\lambda_{L1}\!=\!0$ in Eq.~\eqref{eq:normal-loss}).
Interestingly, this contradicts what one sees when examining the results visually. 
Looking at the reconstructed surfaces reveals that they look more natural and more similar to the ground-truth without $L1$.
A few examples illustrating this are provided in Figures~\ref{fig:normal_data},~\ref{fig:rendered_data}. 
This phenomena is actually not surprising at all. In fact, it is aligned with the recent trends in super-resolution, discussed in Section~\ref{sec:super-resolution}, where perceptual evaluation measures are becoming a common assessment tool. 
Unfortunately, such perceptual measures are not the common evaluation criteria for assessing reconstruction of surface normals.


Finally, we would like to emphasize, that our approach generalizes well to other textures outside our dataset. This can be seen from the results in Figure~\ref{fig:teaser} where two texture images, found online, were fed to our trained network. The reconstructed surface normals are highly detailed and look natural.














==> fig_SR_plane.tex <==
\begin{figure}[t]
		\centering
        \includegraphics[width=\linewidth]{Mechrez_plots_crop.png}
		\vspace*{-0.5cm}
        \caption{\textbf{Perception-distortion evaluation}: Following \cite{blau2017perception} we plot 14 algorithms on the perception-distortion plane. Perception is measured by the NR metric by Ma \etal~\cite{ma2017learning} which is specifically designed for SR quality assessment. Distortion is measured by the common metrics MSE, SSIM~\cite{wang2004image} and MS-SSIM~\cite{wang2003multiscale} and advanced metrics IFC~\cite{sheikh2005information} and VIF~\cite{sheikh2006image}. In four out of five plots, no method appear better then our method on both distortion and perception concurrently. Our method is marked as \textbf{\color{ProcessBlue} Mechrez}.}
		\label{fig:SR_plane}
\end{figure}



==> fig_analysis.tex <==
\begin{figure}[t]
		\centering
		\setlength{\tabcolsep}{.15em}
        \small
        \begin{tabular}{p{.25\linewidth}p{.25\linewidth}cc} 
		\includegraphics[width=\linewidth]{analysis/input_a.png}&
        \includegraphics[width=\linewidth]{analysis/target_b_all.jpg}&
		\includegraphics[width=.25\linewidth]{analysis/L1_a.png}&
		\includegraphics[width=.25\linewidth]{analysis/contextual_a.png}\\
        (a) Noisy input & (b) Clean targets & (c) Cleaned with $L1$ & (d) Cleaned with $\mathcal{L}_{\text{CX}}$
        \end{tabular}
        \vspace*{-0.2cm}
		\caption{\textbf{Robustness to misalignments}: 
        A noisy input image (a) is cleaned via gradient descent, where the target clean images (b) show the same scene, but are not aligned with the input. Optimizing with $L1$ leads to a highly blurred result (c) while optimizing with our contextual loss $\mathcal{L}_{\text{CX}}$ removes the noise nicely (d). This is since $\mathcal{L}_{\text{CX}}$ is robust to misalignments and spatial deformations.
        }
		\label{fig:Analysis}
\end{figure}

==> fig_applications.tex <==
\begin{table}[t]
		\centering
		\setlength{\tabcolsep}{.1em}
        \small
        \begin{tabular}{c l c c c c c} 
         &  &  & \multicolumn{2}{c}{\underline{ \ \ \ \ \ \textbf{Loss function} \ \ \ \ \ }} & & \\
        %
        \textbf{\#} & \textbf{Application}
        & \textbf{Architecture} & \textbf{Proposed} & \textbf{Previous} & \textbf{Paired} & \textbf{Aligned}\\
        \hline
        1& Style transfer  & Optim.~\cite{gatys2016image} & $\mathcal{L}_{\text{CX}}^{target}+\mathcal{L}_{\text{CX}}^{identity}$ 	& 
        $\mathcal{L}_{P} + \mathcal{L}_{Gram}$ &
        \includegraphics[width=.015\linewidth]{v.png} & \includegraphics[width=.015\linewidth]{x.png}
        \\
        \myrowcolour
        2-1& ITIT:one2one & CRN~\cite{chen2017photographic} 	& $\mathcal{L}_{\text{CX}}^{target} + \mathcal{L}_{P}^{coarse}$				& 
        $\mathcal{L}_{P} + \mathcal{L}_{1}$  & \includegraphics[width=.015\linewidth]{v.png} & \includegraphics[width=.015\linewidth]{v.png} \includegraphics[width=.015\linewidth]{x.png}
        \\
        2-2& ITIT:many2one & CRN~\cite{chen2017photographic} 	& 
        $\mathcal{L}_{\text{CX}}^{target}+\mathcal{L}_{\text{CX}}^{identity}$ & 
        $\mathcal{L}_{P} + \mathcal{L}_{1}$  & 
\includegraphics[width=.015\linewidth]{v.png} &  \includegraphics[width=.015\linewidth]{x.png}
		\\
        \myrowcolour
        2-3& ITIT:many2many & CRN~\cite{chen2017photographic} 	& 
        $\mathcal{L}_{\text{CX}}^{target}+\mathcal{L}_{\text{CX}}^{identity}$ & 
        $\mathcal{L}_{P} + \mathcal{L}_{1}$  & 
\includegraphics[width=.015\linewidth]{x.png} & \includegraphics[width=.015\linewidth]{x.png}
        \\
        3& Super-resolution	& SRGAN\cite{ledig2016photo} & $\mathcal{L}_{\text{CX}}^{target}+\mathcal{L}_{GAN}$ & 
        $\mathcal{L}_{P} + \mathcal{L}_{GAN}$  & \includegraphics[width=.015\linewidth]{v.png} & \includegraphics[width=.015\linewidth]{v.png} 
        \\         
        & & & $+\mathcal{L}_{L2}^{coarse}$ & & & \\
        \hline
        \end{tabular}
        \vspace*{0.1cm}
		\caption{\textbf{Applications settings}: A summary of the settings for 5 applications (ITIT=Image-To-Image-Translation).
        We distinguish between paired and unpaired data and between aligned, semi-aligned (x+v) and non-aligned data. 
        Definitions for the loss functions are in the text. \itamar{should we change the order of the methods to match the order of the paper?} 
        }
        \vspace*{-0.5cm}
		\label{tab:applications}
\end{table}

==> fig_inpainting.tex <==
\begin{figure}[t]
	\centering
	\small
        \setlength{\tabcolsep}{.1em}
        \renewcommand{\arraystretch}{0}
        \scriptsize
                %
    \begin{tabular}{ccc  ccc  ccc} 
    \rotatebox[origin=l]{90}{\centering \ \textbf{Original}}&
    \includegraphics[width=.115\linewidth]{inpaint/001_im_gt.png}&
	\includegraphics[width=.115\linewidth]{inpaint/005_im_gt.png}&
    \includegraphics[width=.115\linewidth]{inpaint/078_im_gt.png}&
	\includegraphics[width=.115\linewidth]{inpaint/041_im_gt.png}&
    \includegraphics[width=.115\linewidth]{inpaint/049_im_gt.png}&
	\includegraphics[width=.115\linewidth]{inpaint/050_im_gt.png}&
    \includegraphics[width=.115\linewidth]{inpaint/054_im_gt.png}&
	\includegraphics[width=.115\linewidth]{inpaint/064_im_gt.png}\\
    %
    \hline
    \hline
    \rotatebox[origin=l]{90}{\centering \ \textbf{CE~\cite{pathak2016context}}}&
    \includegraphics[width=.115\linewidth]{inpaint/001_im_default.png}&
    \includegraphics[width=.115\linewidth]{inpaint/005_im_default.png}&
    \includegraphics[width=.115\linewidth]{inpaint/078_im_default.png}&
    \includegraphics[width=.115\linewidth]{inpaint/041_im_default.png}&
    \includegraphics[width=.115\linewidth]{inpaint/049_im_default.png}&
    \includegraphics[width=.115\linewidth]{inpaint/050_im_default.png}&
    \includegraphics[width=.115\linewidth]{inpaint/054_im_default.png}&
    \includegraphics[width=.115\linewidth]{inpaint/064_im_default.png}\\
    %
    \hline
    \hline
    \rotatebox[origin=l]{90}{\centering \ \textbf{\ \ Ours }}&
    \includegraphics[width=.115\linewidth]{inpaint/001_im_run_A0_001_D12_22_0_1_s0_1d0_05__C1.png}&
    \includegraphics[width=.115\linewidth]{inpaint/005_im_run_A0_001_D12_22_0_1_s0_1d0_05__C1.png}&
    \includegraphics[width=.115\linewidth]{inpaint/078_im_run_A0_001_D12_22_0_1_s0_1d0_05__C1.png}&
    \includegraphics[width=.115\linewidth]{inpaint/041_im_run_A0_001_D12_22_0_1_s0_1d0_05__C1.png}&
    \includegraphics[width=.115\linewidth]{inpaint/049_im_run_A0_001_D12_22_0_1_s0_1d0_05__C1.png}&
    \includegraphics[width=.115\linewidth]{inpaint/050_im_run_A0_001_D12_22_0_1_s0_1d0_05__C1.png}&
    \includegraphics[width=.115\linewidth]{inpaint/054_im_run_A0_001_D12_22_0_1_s0_1d0_05__C1.png}&
    \includegraphics[width=.115\linewidth]{inpaint/064_im_run_A0_001_D12_22_0_1_s0_1d0_05__C1.png}\\
	\end{tabular}
    \vspace*{-0.2cm}
    \caption{
		\textbf{Inpainting qualitative results}: Our results compared to CE~\cite{pathak2016context}.  }
        \vspace*{-0.5cm}
	\label{fig:inpaint_results}
\end{figure}


==> fig_inpainting_table.tex <==
\begin{table}
\setlength{\tabcolsep}{.8em}
\centering

\begin{tabular}{l | ccc}
\textbf{Method} & Ma et al.~\cite{ma2017learning} & Zhang et al.~\cite{zhang2018unreasonable}& PSNR \\
\hline
CE~\cite{pathak2016context} (GAN + L2) & 6.86 & & 	25.01\\
Ours (CS + L2-LF) & 7.15 	& & 23.30\\
\end{tabular}

\vspace*{0.1cm}
\caption{\textbf{Quantitative comparison of inpainitng results}: We measure the perceptual quality of our results using two perceptual measurements: Ma et al.~\cite{ma2017learning} and Zhang et al.~\cite{zhang2018unreasonable}. \roey{Our method outperform}  The evaluation is done on Paris street view dataset, with resolution $128\times 128$.}
\label{fig:normal_table}
\end{table}

==> fig_intuition.tex <==
\begin{figure}[t]
\centering
		%\setlength{\tabcolsep}{.15em}
        \small
        \begin{tabular}{cc} 
		\includegraphics[height=2.15cm]{method_img/PQsame_small.png} &
       \includegraphics[height=2.15cm]{method_img/pQqP_small.png}\\
       (a) Similar & (b) Not-similar
       \end{tabular}
       \vspace*{-0.2cm}
	\caption{{\bf Contextual Similarity between images:}
Orange circles represent the features of an image $x$ while the blue triangles represent the features of a GT image $y$. 
The red arrows match each feature in $x$ with its most \emph{contextually similar} (Eq.\eqref{eq:affinity}) feature in $y$.
(a) Images $x$ and $y$ are similar: their features are similarly distributed, and therefore many features in $y$ are matched with similar features in $x$. 
(b) Images $x$ and $y$ are not-similar: the distributions are different, and therefore, many features in $y$ are not matched with any feature in $x$. 
The Contextual loss can be thought of as a weighted sum over the red arrows. 
}
	\label{fig:intuition}
\end{figure}

==> fig_overfit.tex <==
\begin{figure}[t]
		\centering
		\setlength{\tabcolsep}{.1em}
        \scriptsize
        \begin{tabular}{cccc} 
		\includegraphics[width=.24\linewidth]{overfeat/LR.png}&
		\includegraphics[width=.24\linewidth]{overfeat/L1.png}&
		\includegraphics[width=.24\linewidth]{overfeat/DIS.png}&
        \includegraphics[width=.24\linewidth]{overfeat/HR.png}\\
        \includegraphics[width=.24\linewidth]{overfeat/LR1.png}&
		\includegraphics[width=.24\linewidth]{overfeat/L11.png}&
		\includegraphics[width=.24\linewidth]{overfeat/DIS1.png}&
        \includegraphics[width=.24\linewidth]{overfeat/HR1.png}\\
        (a) LR input & (b) Trained with $L2$ & (c) Trained with $\mathcal{L}_{\text{CX}}$ & (d) HR target
        \end{tabular}
        \vspace*{-0.2cm}
		\caption{\textbf{Maintaining natural image statistics in super-resolution}: 
        (b),(c) High-resolution images produced by SRResNet when trained with either $L2$ or $\mathcal{L}_{\text{CX}}$, respectively. Training was done on a single image (see text).
        It can be seen that using the Contextual loss allows hallucination of fine details on the sweater texture, the cracks on the lips, and the facial hair. Conversely, with $L2$, the generated images are blurred ($L1$ results are highly similar, hence, excluded).
        }
		\label{fig:overfit}
\end{figure}

==> fig_power_spectrum.tex <==
\begin{figure}[htb]
		\setlength{\tabcolsep}{.0em}
        \centering
        \scriptsize
        \begin{tabular}{cccccccc}
        \makebox[.143\textwidth]{(a)}&
        \makebox[.143\textwidth]{(b)}&
        \makebox[.143\textwidth]{(c)}&
        \makebox[.143\textwidth]{(d)}&
        \makebox[.143\textwidth]{(e)}&
        \makebox[.143\textwidth]{(f)}&
        \makebox[.143\textwidth]{(g)}\\
        
        \end{tabular}
        \includegraphics[width=\textwidth]{mean_power_spectrum_for_SR.jpg}
		\vspace*{-0.5cm}
        \caption{\textbf{Natural image statistics}: The mean power spectra of images reconstructed by six different super-resolution methods: (a) bicubic (as baseline);  (b) LapSRN~\cite{LapSRN} and (c) SRResNet-MSE~\cite{ledig2016photo} are designed for high PSNR and trained with $L2$ as loss;  In contrast, (d) SRGAN~\cite{ledig2016photo}, (e) EnhanceNet~\cite{sajjadi2017enhancenet}, and, (f) ours, are all trained with GAN and aim for high perceptual quality. 
        (g) The mean power-spectrum of the ground-truth high-resolution images.
        It can be seen that methods aimed at perceptual quality (d,e,f) produce images with more natural power-spectrum than methods aimed at high PSNR (a,b,c).
        The latter lack high-frequencies.
        }
		\label{fig:power_spectrum}
\end{figure}



==> fig_random_projection.tex <==
\definecolor{in}{rgb}{1,    0,    1}
\definecolor{out}{rgb}{1,    0,    1}
\definecolor{tar}{rgb}{0,    1,    0}

\begin{figure}[!h]
		\centering
%        \begin{tabular}{cccc}
%         \multirow{2}{*}{\includegraphics[width=0.3\textwidth,height=4cm]{kde1.jpg}} &
%         \includegraphics[width=0.2\textwidth]{analysis/3-i.png}&
%         \includegraphics[width=0.2\textwidth]{analysis/3-L1.png}&
%         \includegraphics[width=0.2\textwidth]{analysis/3-dis.png}\\
%         &
%         \includegraphics[width=0.2\textwidth]{analysis/4-i.png}&
%         \includegraphics[width=0.2\textwidth]{analysis/4-L1.png}&
%         \includegraphics[width=0.2\textwidth]{analysis/4-dis.png}\\
%         (a) &
%         (a) Initial & (b) Optimized with $L1$ & (c) Optimized with $\mathcal{L}_{\text{CX}}$\\
%         \end{tabular}
        \begin{tabular}{ccc}
        \includegraphics[width=0.2\textwidth]{analysis/3-i.png}&
        \includegraphics[width=0.2\textwidth]{analysis/3-L1.png}&
        \includegraphics[width=0.2\textwidth]{analysis/3-dis.png}\\
        \includegraphics[width=0.2\textwidth]{analysis/4-i.png}&
        \includegraphics[width=0.2\textwidth]{analysis/4-L1.png}&
        \includegraphics[width=0.2\textwidth]{analysis/4-dis.png}\\
        (a) Initial & \ \ (b) Optimized with $L1$ & \ \ \ (c) Optimized with $\mathcal{L}_{\text{CX}}$\\
        \end{tabular}
        %
        %
        %
%         \animategraphics[autoplay,loop,width=0.99\linewidth]{1}{analysis/rp-}{1}{2} 
% 		\includegraphics[width=0.24\textwidth]{analysis/DIS_project2_0.png}
%         \includegraphics[width=0.24\textwidth]{analysis/DIS_project4_0.png}
%         \includegraphics[width=0.24\textwidth]{analysis/DIS_project7_0.png}
%         \includegraphics[width=0.24\textwidth]{analysis/DIS_project8_0.png}~
        
%         \includegraphics[width=0.24\textwidth]{analysis/DIS_project2_Final.png}
%         \includegraphics[width=0.24\textwidth]{analysis/DIS_project4_Final.png}
%         \includegraphics[width=0.24\textwidth]{analysis/DIS_project7_Final.png}
%         \includegraphics[width=0.24\textwidth]{analysis/DIS_project8_Final.png}~
        
%         \includegraphics[width=0.24\textwidth]{analysis/L1_project2_0.png}
%         \includegraphics[width=0.24\textwidth]{analysis/L1_project4_0.png}
%         \includegraphics[width=0.24\textwidth]{analysis/L1_project7_0.png}
%         \includegraphics[width=0.24\textwidth]{analysis/L1_project8_0.png}~
        
%         \includegraphics[width=0.24\textwidth]{analysis/L1_project2_Final.png}
%         \includegraphics[width=0.24\textwidth]{analysis/L1_project4_Final.png}
%         \includegraphics[width=0.24\textwidth]{analysis/L1_project7_Final.png}
%         \includegraphics[width=0.24\textwidth]{analysis/L1_project8_Final.png}~
        \vspace*{-0.2cm}
		\caption{\textbf{Minimizing the difference between distributions}: Random projections of image patches onto 2D illustrate the distribution of patches in an image.                
        The projection of the patches of the \textbf{\textcolor{tar}{target}}  are in \textbf{\textcolor{tar}{green}}. The \textbf{\textcolor{in}{input}} and the final \textbf{\textcolor{out}{output}} are both in \textbf{\textcolor{out}{Magenta}}.  
        When two projections agree, they overlap and the color turns to \textbf{Black}.
        We compare between the target image and (a) the input image, (b) the output after optimization with $L1$, and, (c) the output after optimizing with $\mathcal{L}_{\text{CX}}$ (more details in the text).
        Optimizing with $\mathcal{L}_{\text{CX}}$ reduces the outliers and yields high correlation (more black) with the target, while using $L1$ barely reduces the gap between the densities.}
		\label{fig:random}
\end{figure}

==> fig_support.tex <==
\begin{figure}[t]
		\setlength{\tabcolsep}{.15em}
        \centering
        \scriptsize
        \begin{tabular}{ccc}
        Small spatial support&
        Large spatial support&
        Statistical support\\
        \includegraphics[width=0.25\textwidth]{support/a3.jpg}&
        \includegraphics[width=0.25\textwidth]{support/b3.jpg}&
        \includegraphics[width=0.25\textwidth]{support/c3.jpg}
        \end{tabular}
		\vspace*{-0.2cm}
        \caption{\textbf{Importance of spatial support during training:} In order to be able to reconstruct specific pattern, illustrate by the lightning, the spatial support should include distant pixels of the same pattern. The pixel $p_1$ is computed from the influencing region in the spatial support $\Omega_1$, while the pixel $p_2$ cannot be calculated since the supporting area $\Omega_2$ does not contain the necessary information. This improve when the spatial support is larger. Our solution takes the entire image as the support (context) by utilize the statistical approach of the Contextual loss. Here we illustrate for image SR, with out the loss of generality, same insight is true for all image restoration problems. Similar idea was shown in \cite{iizuka2017globally} during test time.}
\label{fig:support}
\end{figure}

==> priors.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Priors in Image Restoration}
\roey{
From vedaldi~\cite{ulyanov2017deep}
Overall, the prior imposed by deep ConvNets and investigated in this work seems to be highly related to selfsimilarity-based and dictionary-based priors. Indeed, as the weights of the convolutional filters are shared across the entire spatial extent of the image this ensures a degree of self-similarity of individual patches that a generative ConvNet can potentially produce. 
\\
GAN-based methods SRGAN [18] and EnhanceNet [27] (not shown in the comparison) intelligently
hallucinate fine details of the image, which is impossible
with our method that uses absolutely no information about
the world of HR images.
\\


The deep image prior utilizes context of the image and interpolates the unknown region with textures from the known part. Such behaviour highlights the relation between the deep image prior and traditional self-similarity priors.
\\

from \cite{lefkimmiatis2017non} 
the resulting models are local ones and do not take into account the inherent non-local self-similarity property of natural images
\\

from irani~\cite{shocher2017zero}
The recurrence of small pieces of information (e.g.,
small image patches) across scales of a single image, was shown to be a very strong property of natural images
\\

Some text ideas: 
same distribution is same as use all the patches in the generated image. 

The algorithms are comparable in smooth homogeneous regions. in texture regions with fine details, the PSNR/L2 methods cause blur, while perceptual methods create fine details which are not aligned to the GT. Respectively, the former results with higher error when comparing pixel-to-pixel, yet, a human observer is not sensitive to this miss-alignment and usually prefer real texture over the smooth regions. 
}

==> training.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Training CNNs to generate natural statistics}
\label{sec:method}

\input{fig_CX.tex}

\subsubsection{Proposed Framework:\ \ \  }
Our approach is very simple, as depicted in Figure~\ref{fig:CX}.
To train a generator network $G$ we use pairs of source $s$ and target $t$ images. The network outputs an image $G(s)\!=\!x$, that should be as similar as possible to the target $t$.
To measure the similarity we extract from both $x$ and $t$ dense deep features (e.g., using VGG19~\cite{simonyan2014very}), and compare their distributions via the Contextual loss, recently proposed by Mechrez et al.~\cite{mechrez2018contextual}.
While they suggested it for comparing images that are not spatially aligned, we show that it pertains further properties, that render it a good fit for our purposes.
We next briefly describe the Contextual loss, and then discuss its statistical properties. For detailed definition we refer the reader to~\cite{mechrez2018contextual}.




% \roey{cite  regarding power spectrum van1996modelling, Cite  Salimans (Improved Techniques for Training GANs) regarding difficulty in training GANs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Review of the Contextual Loss:\ \ \ }
%\vspace*{-0.1cm}

% For training a generator network the contextual loss is defined based on the contextual similarity of Eq.\eqref{eq:CS}.
% Let $x$ and $y$ be two images to be compared.
% Corresponding set of features are extracted from the images by passing them through a perceptual network $\Phi$  (classically $\Phi$ is VGG19~\cite{simonyan2014very}).
% Let $\Phi^l(x)$, $\Phi^l(y)$ denote the feature maps extracted from layer $l$ of the perceptual network $\Phi$ of the images $x$ and $y$, respectively.


% The Contextual loss $\mathcal{L}_{\text{CX}}(x,y)$ is a distance between a pair of images $x$ and $y$. Each image is represented as a set of high-dimensional points (features), and the distance between the two point sets is considered to be small if they have similar underlying distributions. Subsequently, $\mathcal{L}_{\text{CX}}(x,y)$ is a distance measure that ask whether two images have the same inner statistics. 

% Since this is a statistical loss it measure the similarity between two point sets, i.e. when the points corresponding to two images are sampled from similar distributions -- the images are consider similar.  Conversely, when the images are not similar, the points are sampled from different distributions, and many features would have no similar one in the other image. In other words, this idea can be define as a similarity measure that ask whether two images have the same inner statistics.
%Next, We briefly formulate the Contextual loss (CX), for detail definition we refer the reader to Mechrez et al.~\cite{mechrez2018contextual}.
%
\roey{here we call the target image y and before we named it t, not sure what is best maybe change all y with t? although x and t is a bit odd. }
Given a generated image $x$ and a target image $y$ each is represented as a collection of points (e.g., VGG19 features~\cite{simonyan2014very} or vectorized RGB patches): $X\!=\!\{x_i\}$ and $Y\!=\!\{y_j\}$. It is assumed that $|Y|\!=\!|X|\!=\!N$ (and sample $N$ points from the bigger set when $|Y|\!\neq\!|X|$). 
Let $A_{ij}$ denote the affinity between $x_i$ and $y_j$.
The Contextual loss is defined as:
%
\begin{empheq}[]{equation}
\label{eq:CX}
\mathcal{L}_{\text{CX}}(x,y) = -\log \bigg( \, \frac{1}{N}\sum_{j} { \max_{i}{\text{A}_{ij}} }   \, \bigg)
\end{empheq} 

The affinities $A_{ij}$ are obtained by first computing the Cosine distance $d_{ij}$ between all pairs $x_i$,$y_j$.
%\footnote{
%$d_{ij}=(1-\frac{(x_i-\mu_y) \cdot  (y_j-\mu_y)}{||x_i-\mu_y||_2|| y_j-\mu_y||_2})$ where $\mu_y$$=\frac{1}{N}\sum_{j}{y_j}$.}.
%
Points $x_i$ and $y_j$ are considered \emph{similar} when $d_{ij}\!\gg\!d_{ik}, \forall k\!\neq\!j$.
To capture this the distances are normalized: $\hat{d}_{ij}\!=\!{d_{ij}}/({\min_{k}{d_{ik}} + \epsilon})$ (for a small value $\epsilon$), and then the pairwise affinities $A_{ij}$ are computed as: $\text{A}_{ij} ={e^{\left( {1 - \hat{d}_{ij}}/{h} \right)}}/{\sum_{k}{e^{\left( {1 - \hat{d}_{ik}}/{h} \right)}}}$, where $h\!>\!0$ is a band-width parameter.
%
%Given $a_{ij}$, we can define the key component of the loss -- an affinity matrix $A_{ij}$ between points $x_i\!\in\!X$ and points $y_j\!\in\!Y$:
%
% \begin{equation}
% \label{eq:affinity}
% 	\text{A}_{ij} =\frac{e^{\left( {1 - a_{ij}}/{h} \right)}} {\sum_{k}{e^{\left( {1 - a_{ik}}/{h} \right)}}}
% \end{equation}

 

It can be seen from Eq.~\eqref{eq:CX} that the loss is minimized when every feature $y_j$ of the target image has a matching feature $x_n$ in the generated image, with high affinity between them, that is:
%
\begin{align}
\label{eq:Anj}
A_{nj} = 
\begin{cases}
  \approx 1 & \text{if\ \ } dist(x_n,y_j) \ll dist(x_k,y_j) \mbox{\ \ } \forall k\neq n\\    
  \approx 0 &  \text{otherwise}
\end{cases}
\end{align}




%In image transformation tasks we train a network $G$ to map a given source image $s$ into an output image $G(s)$. To demand similarity between the generated image and the target using CX as the objective we notate: $\mathcal{L}_{\text{CX}}(G(s),t)$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Contextual Similarity Between Images}
% %\vspace*{-0.1cm}
% %



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{The Contextual Similarity:}

% To calculate the similarity between the images we find for each feature $y_j$  the feature $x_i$ that is most similar to it, and then sum the corresponding feature similarity values over all $y_j$. 
% Formally, the contextual similarity between images is defined as:
% %
% \begin{equation}
%     \label{eq:CS}
% 	\text{CS}(X,Y) = \frac{1}{N}\sum_{j} { \max_{i}{\text{A}_{ij}} }
% \end{equation}
% %
% where $\text{A}_{ij}$, to be defined next, is the similarity between features $x_i$ and $y_j$.

% The global image context is incorporate via the similarity $\text{A}_{ij}$ between features.
% Specifically, feature $x_i$ is contextually similar to feature $y_j$ if it is significantly closer to it than to all other features in $Y$. 
% When this is not the case, i.e., $x_i$ is not closer to any particular $y_j$, then its contextual similarity to all $y_j$ should be low.
% This approach is robust to the scale of the distances, e.g., if $x_i$ is far from all $y_j$ then $\text{A}_{ij}$ will be low $\forall j$ regardless of how far apart $x_i$ is. 












